Using a one dimensional parabolic model of the full-batch loss to estimate learning rates during training

A fundamental challenge in Deep Learning is to find optimal step sizes for stochastic gradient descent automatically. In traditional optimization, line searches are a commonly used method to determine step sizes. One problem in Deep Learning is that finding appropriate step sizes on the full-batch loss is unfeasibly expensive. Therefore, classical line search approaches, designed for losses without inherent noise, are usually not applicable. Recent empirical findings suggest, inter alia, that the full-batch loss behaves locally parabolically in the direction of noisy update step directions. Furthermore, the trend of the optimal update step size changes slowly. By exploiting these and more findings, this work introduces a line-search method that approximates the full-batch loss with a parabola estimated over several mini-batches. Learning rates are derived from such parabolas during training. In the experiments conducted, our approach is on par with SGD with Momentum tuned with a piece-wise constant learning rate schedule and often outperforms other line search approaches for Deep Learning across models, datasets, and batch sizes on validation and test accuracy. In addition, our approach is the first line search approach for Deep Learning that samples a larger batch size over multiple inferences to still work in low-batch scenarios.

==> labpal/batch_size_10_best.tex <==
\begin{figure}[h!]
	\tikzsetfigurename{labpal_opt_comparison_bs10_best}
	\centering
	\def\scale{0.4}
	
	\begin{tabular}{ c c c}	
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_ResNet-20_learning_rate.pgf"}}&	
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_MobileNet-V2_learning_rate.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_DenseNet-121_learning_rate.pgf"}}\\
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_ResNet-20_training_loss.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_MobileNet-V2_training_loss.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_DenseNet-121_training_loss.pgf"}}\\
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_ResNet-20_validation_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_MobileNet-V2_validation_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_DenseNet-121_validation_accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_ResNet-20_test_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_MobileNet-V2_test_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_best/CIFAR-10_DenseNet-121_test_accuracy.pgf"}}
	\end{tabular}
	\caption{Performance comparison of several models on CIFAR-10 with \textbf{batch size 10}. For the LABPAL approaches only the noise factor is adapted according to equation \ref{eq_noise_factor1}.  For all other approaches, a grid search is performed to find the best hyperparameters for this scenario. (see Appendix \ref{app_hyperparams}). In comparison to Figure \ref{labpal_fig_opt_comparison_bs10_same}, now,  the LABPAL approaches perform competitive on the training loss and surpass the other approaches on validation and test accuracy. PLS plots are incomplete since the training failed after some steps.} 
	\label{labpal_fig_opt_comparison_bs10_best}
\end{figure}

==> labpal/batch_size_10_same.tex <==
\begin{figure}[h!]
	\tikzsetfigurename{labpal_opt_comparison_bs32}
	\centering
	\def\scale{0.4}
	
	\begin{tabular}{ c c c}
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_ResNet-20_learning_rate.pgf"}}&	
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_MobileNet-V2_learning_rate.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_DenseNet-121_learning_rate.pgf"}}\\
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_ResNet-20_training_loss.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_MobileNet-V2_training_loss.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_DenseNet-121_training_loss.pgf"}}\\
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_ResNet-20_validation_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_MobileNet-V2_validation_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_DenseNet-121_validation_accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_ResNet-20_test_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_MobileNet-V2_test_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison_low_batch/plots_same/CIFAR-10_DenseNet-121_test_accuracy.pgf"}}

	\end{tabular}
	\caption{Performance comparison of several models on CIFAR-10 with \textbf{batch size 10}. \textbf{The same hyperparameters are used as for batch size 128} (see Figure \ref{labpal_fig_optimizer_comparison_cifar10}). PAL and PLS fail in this scenario. The LABPAL approaches work well in the beginning but fail to estimate well learning rates later; this is solved in Figure \ref{labpal_fig_opt_comparison_bs10_best}. Interestingly, they still achieve competitive validation and test accuracies.} 
	\label{labpal_fig_opt_comparison_bs32}
\end{figure}

==> labpal/figure_strategy_metrics2.tex <==

\begin{figure}[b!]
	%\centering
	\def\scale{0.362}
	\def\basis{10e-5}
	%\scalebox{1.0}{
	%\input{"\figureTwoDataPath CIFAR10_mom0_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
	
	\begin{tabular}{ c c c }
		\scalebox{\scale}{\input{"\figureTwoDataPath CIFAR10_mom0_resnet20_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/step_step.pgf"}}&\hspace{-0.25cm}
		%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library	
		\scalebox{\scale}{\input{"\figureTwoDataPath
		CIFAR10_mom0_resnet20_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/improvements_step_accumulated.pgf"}}&\hspace{-0.25cm}
		\scalebox{\scale}{\input{"\figureTwoDataPath CIFAR10_mom0_resnet20_augment_result/statistics_plots/bs_128_bs_ori_128_sgd_lrs_[0.05]_pal_mus_[0.1]_ri_100_c_apal_0.9_ori_sgd_lr_0.1/fb_min_step_ratio.pgf"}}
	\end{tabular}

	\caption{Several metrics to compare update step strategies on the  full-batch losses along 10000 lines measured by \cite{line_analysis}: 1. update step sizes, 2. the accumulated loss improvement per step given as:  $l(0)-l(s_{upd})$ where $s_{upd}$ is the update step of a specific optimizer. Note that this is the locally optimal improvement to the minimum of the full-batch loss along a line. Average smoothing with a kernel size of 25 is applied. The right plot shows almost proportional behavior between the optimal update step and the directional derivative (negative gradient norm) of the direction defining mini-batch loss. The LABPAL\&SGD version of our approach is added and performs almost optimal. The figure is taken with permission from \cite{line_analysis}.}
	\label{fig_strategy_metrics}
\end{figure}

%\begin{tikzpicture}
%	\def\basis{10e-6}
%	
%	%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library
%	\pgfplotsset
%	{
%		y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		yticklabel style={/pgf/number format/.cd,int detect,precision=2},
%	}
%pdflatex --enable-write18 -shell-escape -interaction=nonstopmode %.tex

==> labpal/optimizer_comparison.tex <==
\begin{figure}[t!]
	\centering
	\def\scale{0.362}
	\def\basis{10e-5}
	%\scalebox{1.0}{
	%\input{"\figureTwoDataPath CIFAR10_mom0_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
	
	\begin{tabular}{ c c c }
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-20_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-20_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-20_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_DenseNet-121_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_DenseNet-121_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_DenseNet-121_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_MobileNet-V2_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_MobileNet-V2_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_MobileNet-V2_validation accuracy.pgf"}}\\
		
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_ResNet-20_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_ResNet-20_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_ResNet-20_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_DenseNet-121_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_DenseNet-121_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_DenseNet-121_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_MobileNet-V2_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_MobileNet-V2_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-100_MobileNet-V2_validation accuracy.pgf"}}\\
		
		
		

	\end{tabular}
	
	\caption{Several metrics to compare update step strategies: 1. update step sizes, 2. the distance to the minimum of the full batch loss ($s_{opt}-s_{upd}$), which is the optimal update step from a local perspective. 3. the loss improvement per step given as:  $l(0)-l(s_{upd}))$ where $s_{upd}$ is the update step of a strategy. Average smoothing with a kernel size of 25 is applied. The right lower plot shows almost proportional behavior between $s_{opt}$ and the directional derivative of the direction defining mini-batch loss. }
	\label{fig_optimizer_comparison}
\end{figure}





\begin{figure}[t!]
	\centering
	\def\scale{0.362}
	\def\basis{10e-5}
	%\scalebox{1.0}{
	%\input{"\figureTwoDataPath CIFAR10_mom0_resnet20_augment_result/statistics_plots/distance_matrix.pgf"}}\\
	
	\begin{tabular}{ c c c }
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_ResNet-20_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_ResNet-20_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_ResNet-20_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_DenseNet-121_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_DenseNet-121_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_DenseNet-121_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_MobileNet-V2_step size.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_MobileNet-V2_training loss.pgf"}}&
		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/SVHN_MobileNet-V2_validation accuracy.pgf"}}\\
		
		
		
	\end{tabular}
	
	\caption{Several metrics to compare update step strategies: 1. update step sizes, 2. the distance to the minimum of the full batch loss ($s_{opt}-s_{upd}$), which is the optimal update step from a local perspective. 3. the loss improvement per step given as:  $l(0)-l(s_{upd}))$ where $s_{upd}$ is the update step of a strategy. Average smoothing with a kernel size of 25 is applied. The right lower plot shows almost proportional behavior between $s_{opt}$ and the directional derivative of the direction defining mini-batch loss. }
	\label{fig_optimizer_comparison2}
\end{figure}

%\begin{tikzpicture}
%	\def\basis{10e-6}
%	
%	%https://tex.stackexchange.com/questions/447795/pgf-fpu-ill-formatted-floating-point-number-using-shapes-symbols-library
%	\pgfplotsset
%	{
%		y coord trafo/.code={\begingroup\pgfmathparseFPU{symlog(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		y coord inv trafo/.code={\begingroup\pgfmathparseFPU{symexp(#1,\basis)}\pgfmathsmuggle\pgfmathresult\endgroup},
%		yticklabel style={/pgf/number format/.cd,int detect,precision=2},
%	}
%pdflatex --enable-write18 -shell-escape -interaction=nonstopmode %.tex

==> labpal/optimizer_comparison_cifar10.tex <==

\begin{figure}[t!]
	\centering
	\def\scale{0.45}
%	\begin{tabular}{ c c c}
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_DenseNet-121_step size.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_DenseNet-121_training loss.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_DenseNet-121_validation accuracy.pgf"}}\\
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_MobileNet-V2_step size.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_MobileNet-V2_training loss.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_MobileNet-V2_validation accuracy.pgf"}}\\
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-20_step size.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-20_training loss.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-20_validation accuracy.pgf"}}\\
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-34_step size.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-34_training loss.pgf"}}&
%		\scalebox{\scale}{\input{"/home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/Evaluation/optimizer_step_plots/plots/CIFAR-10_ResNet-34_validation accuracy.pgf"}}\\		
%	\end{tabular}
	
	%\scalebox{0.55}{
	%\input{"//home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/line_plots/bs_128_bs_ori_128_sgd_lrs_[0.01]_pal_mus_[0.1]_ri_50_c_apal_0.9_ori_sgd_lr_0.1/sgd_pal_line_10.pgf"}\hspace{-0.2cm}
	%\input{"//home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/line_plots/bs_128_bs_ori_128_sgd_lrs_[0.01]_pal_mus_[0.1]_ri_50_c_apal_0.9_ori_sgd_lr_0.1/sgd_pal_line_3000.pgf"}\hspace{-0.2cm}
	%\input{"//home/mutschler/PycharmProjects/LineSearchExperiments_Pytorch/LineEvaluation/CIFAR10_mom09_resnet20_augment_result/line_plots/bs_128_bs_ori_128_sgd_lrs_[0.01]_pal_mus_[0.1]_ri_50_c_apal_0.9_ori_sgd_lr_0.1/sgd_pal_line_3200.pgf"}\hspace{-0.2cm}
	%}
	
	\caption{TODO}
	
	\label{optimizer_comparison_cifar10}
\end{figure}

==> labpal/performance_comparison_fashion_mnist.tex <==
\begin{figure}[h!]
	\centering
	\def\scale{0.42}
	
	\begin{tabular}{ c c}	
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-Conv_learning rate.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-FC_learning rate.pgf"}}\\
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-Conv_training loss.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-FC_training loss.pgf"}}\\
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-Conv_validation accuracy.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-FC_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-Conv_test accuracy.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/Fashion-MNIST/Fashion-MNIST_3-Layer-FC_test accuracy.pgf"}}
	\end{tabular}
	\caption{Fashion MNIST} 
\end{figure}

==> labpal/performance_comparison_imagenet.tex <==
\begin{figure}[h!]
	\tikzsetfigurename{labpal_optimizer_comparison_imagenet}
	\centering
	\def\scale{0.6}
	
	\begin{tabular}{ c c }	
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison/IMAGENET/ImageNet_MobileNet-V3_learning_rate.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison/IMAGENET/ImageNet_MobileNet-V3_training_loss.pgf"}}\\
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison/IMAGENET/ImageNet_MobileNet-V3_validation_accuracy.pgf"}}&
		\scalebox{\scale}{\input{"labpal/figure_data/performance_comparison/IMAGENET/ImageNet_MobileNet-V3_test_accuracy.pgf"}}\\
	\end{tabular}
		\caption{Performance comparison of top 1 error on \textbf{IMAGENET} of our approach LABPAL in the SGD and NSGD variants against SLS and SGD. Optimal hyperparameters are found with an elaborate grid search. Optimal hyperparameters found with a detailed grid search for CIFAR-10 are reused. Our approaches challenge the other approaches on training loss and test accuracy. SLS fails shortly after the beginning of the training due to too high estimated learning rates. For LABPAL the  adaptation factor $\epsilon$ introduced in Section \ref{labpal_sec_low_batch_size} is applied.} 
	\label{labpal_fig_optimizer_comparison_imagenet}
\end{figure}

==> labpal/performance_comparison_mnist.tex <==
\begin{figure}[h!]
	\centering
	\def\scale{0.42}
	
	\begin{tabular}{ c c}	
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-Conv_learning rate.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-FC_learning rate.pgf"}}\\
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-Conv_training loss.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-FC_training loss.pgf"}}\\
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-Conv_validation accuracy.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-FC_validation accuracy.pgf"}}\\
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-Conv_test accuracy.pgf"}}&
		\scalebox{\scale}{\input{"figure_data/performance_comparison/MNIST/MNIST_3-Layer-FC_test accuracy.pgf"}}
	\end{tabular}
	\caption{FMNIST} 
\end{figure}
